Towards Adaptive Human-centric Video Anomaly Detection: A Comprehensive Framework and A New Benchmark

Human-centric Video Anomaly Detection (VAD) aims to identify human behaviors that deviate from normal. At its core, human-centric VAD faces substantial challenges, such as the complexity of diverse human behaviors, the rarity of anomalies, and ethical constraints. These challenges limit access to high-quality datasets and highlight the need for a dataset and framework supporting continual learning. Moving towards adaptive human-centric VAD, we introduce the HuVAD (Human-centric privacy-enhanced Video Anomaly Detection) dataset and a novel Unsupervised Continual Anomaly Learning (UCAL) framework. UCAL enables incremental learning, allowing models to adapt over time, bridging traditional training and real-world deployment. HuVAD prioritizes privacy by providing de-identified annotations and includes seven indoor/outdoor scenes, offering over 5x more pose-annotated frames than previous datasets. Our standard and continual benchmarks, utilize a comprehensive set of metrics, demonstrating that UCAL-enhanced models achieve superior performance in 82.14% of cases, setting a new state-of-the-art (SOTA). The dataset can be accessed at https://github.com/TeCSAR-UNCC/HuVAD.

==> sec/Annotation.tex <==
\section{Annotation Methodology}
\label{sec:annotation}

\subsection{Anomaly Annotation}

The HuVAD dataset has undergone manual anomaly annotation to guarantee optimal precision. Each frame was labeled and reviewed by at least three different individuals, with random testing conducted to ensure label consistency and accuracy. Anomalous behaviors defined in Section \ref{sec:data_collection}, are considered abnormal for C0 to C5 cameras, while any other typical daily activities are classified as normal. For CSC, actions outlined in Section \ref{sec:data_collection} are deemed normal if conducted during controlled training sessions and considered abnormal otherwise to accurately represent real-world scenarios. \hl{This dataset offers detailed annotations, including both frame-level anomaly labels and spatial information in the form of anomaly region masks. These masks provide precise bounding boxes that localize the regions where anomalies occur, enabling a more granular analysis of the spatial extent of the anomalous events. According to the standard setup used in unsupervised and semi-supervised video anomaly detection (VAD) methods, the primary objective is to distinguish between normal and anomalous events, without the need to specify particular activity classes. Consequently, these methods do not typically include class-specific activities in common benchmark datasets, such as SHT} \cite{liu2018future}, IITB \cite{rodrigues2020multi}, CHAD \cite{danesh2023chad}, and NWPU \cite{Cao_2023_CVPR}. \hl{For this reason, we adopt the same labeling strategy, focusing on the normal vs. anomalous distinction without class-specific annotations.}

\subsection{Person Annotation}

\label{sec:person_anno}
% In real-world applications, anomaly detection models rely on algorithmically extracted data and not manual person annotations. To simulate this, we used models to extract human annotations, incorporating model noise into the data for more realistic benchmarking.
In real-world applications, anomaly detection models rely on algorithmically extracted data rather than manual person annotations. To simulate this, we used models to extract human annotations. \hl{However, to minimize noise while maintaining algorithmic extraction, we employed a semi-automated approach for generating person annotations. Algorithms first extracted the data, followed by manual verification by annotators to ensure accuracy and alignment. Discrepancies in bounding boxes, person IDs, and pose annotations were manually corrected. This hybrid approach balances the efficiency of automation with the precision of human oversight.}

\subsubsection{Bounding Boxes Annotations} are rectangular areas that identify and enclose the position of a detected object/human. The bounding boxes are included in the annotations and utilized in later stages for human pose estimation and tracking. HuVAD utilizes YOLOv8 \cite{yolov8_ultralytics}, a SotA deep learning model for object detection.

\subsubsection{Person ID Annotations} 
enables the temporal analysis necessary for detecting subtle or complex anomalies for VAD. HuVAD uses ByteTrack \cite{zhang2022bytetrack}, a tracking algorithm that employs byte cost and a Kalman filter to efficiently track objects, handling occlusions and preserving identities.


\subsubsection{Human Pose Annotations}
refers to the spatial configuration of human body parts, represented as a set of keypoints enabling the precise analysis of body movements. HuVAD utilizes HRNet \cite{sun2019deep} for human pose estimation. The extracted poses are in the COCO17 \cite{lin2014microsoft} keypoint format. To improve the quality of pose annotations, linear interpolation is used to fill in missing poses. A 15-frame window is used for data smoothing, and interpolated poses are marked with a null visibility field to allow for their optional exclusion from analyses.



% \subsection{Annotation Smoothing}

% Given that the person annotations described in Section \ref{sec:person_anno} are extracted using an amalgam of models, instances may arise where, despite the presence of a person in the scene, their pose data is missing. To enhance the quality of these annotations, we leverage the premise that human movement is relatively slow, particularly in the context of data captured at 30 frames per second. This assumption underpins the rationale for employing linear interpolation to fill in missing annotations. A window size of 15 frames or half a second is selected for data smoothing and the visibility field of interpolated poses is assigned a null value. This designation facilitates the optional exclusion of these interpolated data points from analyses, should researchers wish to focus solely on directly observed poses.

==> sec/Evaluation_protocol.tex <==
\section{Evaluation Protocols}

\begin{table*}[]
% \small
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccc|ccccc@{}}
\toprule\toprule
\textbf{Model} & \textbf{AUC-ROC} & \textbf{AUC-PR} & \textbf{EER} & \textbf{10ER} & \textbf{Model} & \textbf{AUC-ROC} & \textbf{AUC-PR} & \textbf{EER} & \textbf{10ER} \\ \midrule
\multicolumn{5}{c|}{\textbf{C0}} & \multicolumn{5}{c}{\textbf{C1}} \\ \midrule
\multicolumn{1}{c|}{\textbf{MPED-RNN }} & \textbf{79.57} & {\underline{46.76}} & \textbf{0.26} & \textbf{0.37} & \multicolumn{1}{c|}{\textbf{MPED-RNN }} & \textbf{83.57} & {\underline{53.62}} & \textbf{0.22} & \textbf{0.39} \\
\multicolumn{1}{c|}{\textbf{GEPC }} & 59.07 & 28.00 & 0.44 & 0.71 & \multicolumn{1}{c|}{\textbf{GEPC }} & 56.27 & 23.20 & 0.45 & 0.78 \\
\multicolumn{1}{c|}{\textbf{STG-NF }} & 58.96 & \textbf{83.45} & 0.46 & 0.84 & \multicolumn{1}{c|}{\textbf{STG-NF }} & 47.82 & \textbf{78.31} & 0.52 & 0.89 \\
\multicolumn{1}{c|}{\textbf{TSGAD }} & {\underline{ 64.18}}& 31.93& {\underline{0.40}}& {\underline{ 0.66}}& \multicolumn{1}{c|}{\textbf{TSGAD }} & {\underline{68.88}}& 39.02& {\underline{0.35}}& {\underline{0.72}}\\ \midrule
\multicolumn{5}{c|}{\textbf{C2}} & \multicolumn{5}{c}{\textbf{C3}} \\ \midrule
\multicolumn{1}{c|}{\textbf{MPED-RNN }} & \textbf{73.36} & {\underline{47.66}} & \textbf{0.32} & \textbf{0.57} & \multicolumn{1}{c|}{\textbf{MPED-RNN }} & \textbf{83.62} & {\underline{63.87}} & \textbf{0.23} & \textbf{0.42} \\
\multicolumn{1}{c|}{\textbf{GEPC }} & 55.09 & 30.13 & 0.45 & 0.79 & \multicolumn{1}{c|}{\textbf{GEPC }} & 52.40 & 27.09 & 0.50 & 0.77\\
\multicolumn{1}{c|}{\textbf{STG-NF }} & 51.06 & \textbf{74.20} & 0.49 & 0.94 & \multicolumn{1}{c|}{\textbf{STG-NF }} & 49.15 & \textbf{74.10} & 0.50 & 0.90 \\
\multicolumn{1}{c|}{\textbf{TSGAD }} & {\underline{ 62.81}}& 35.53& {\underline{ 0.39}}& {\underline{ 0.73}}& \multicolumn{1}{c|}{\textbf{TSGAD }} & {\underline{ 54.64}}& 24.25& {\underline{ 0.48}}& \underline{0.76}\\ \midrule
\multicolumn{5}{c|}{\textbf{C4}} & \multicolumn{5}{c}{\textbf{C5}} \\ \midrule
\multicolumn{1}{c|}{\textbf{MPED-RNN }} & {\underline{ 74.59}} & {\underline{ 44.55}} & \underline{0.29}& \textbf{0.31}&
\multicolumn{1}{c|}{\textbf{MPED-RNN }} & \textbf{79.23} & {\underline{ 49.09}} & \textbf{0.27} & \textbf{0.41} \\
\multicolumn{1}{c|}{\textbf{GEPC }} & 72.44 & 30.71 & \underline{0.29}& 0.99 &\multicolumn{1}{c|}{\textbf{GEPC }} & 66.05 & 33.04 & \underline{0.36}& {\underline{ 0.56}} \\
\multicolumn{1}{c|}{\textbf{STG-NF }} & 72.24 & \textbf{93.95} & {\textbf{ 0.28}}& {\underline{ 0.71}} & \multicolumn{1}{c|}{\textbf{STG-NF }} & 56.48 & \textbf{82.36} & 0.46 & 0.96 \\
\multicolumn{1}{c|}{\textbf{TSGAD }} & \textbf{75.11}& 37.13& {\textbf{0.28}}& 1.00 & \multicolumn{1}{c|}{\textbf{TSGAD }} & {\underline{ 67.15}}& 35.20& { 0.37}& 0.57\\ \midrule
\multicolumn{5}{c|}{\textbf{CSC}} & \multicolumn{5}{c}{\textbf{Combined}} \\ \midrule
\multicolumn{1}{c|}{\textbf{MPED-RNN }} & 56.85 & 37.13 & {\underline{ 0.43}} & \textbf{0.69} &
\multicolumn{1}{c|}{\textbf{MPED-RNN }} & \textbf{76.05} & {\underline{ 42.83}} & \textbf{0.28} & \textbf{0.49} \\
\multicolumn{1}{c|}{\textbf{GEPC }} & {\underline{ 58.32}} & {\underline{ 41.09}} & \textbf{0.42} & \underline{0.86}&
\multicolumn{1}{c|}{\textbf{GEPC }} & 62.25 & 28.62 & 0.41 & 0.67 \\
\multicolumn{1}{c|}{\textbf{STG-NF }} & 53.60 & \textbf{66.28} & 0.47 & 0.92 &
\multicolumn{1}{c|}{\textbf{STG-NF }} & 57.57 & \textbf{83.77} & 0.46 & 0.90 \\
\multicolumn{1}{c|}{\textbf{TSGAD }} & \textbf{58.91}& 43.28& \underline{0.43}& {\underline{ 0.86}}&
\multicolumn{1}{c|}{\textbf{TSGAD }} & {\underline{ 68.00}}& 34.61& {\underline{ 0.36}}& {\underline{ 0.64}}\\ \bottomrule \bottomrule
\end{tabular}%
% }

\caption{Benchmarking SotA pose-based models (with available code) on HuVAD. We have used MPED-RNN \cite{morais2019learning}, GEPC \cite{markovitz2020graph}, STG-NF \cite{Hirschorn_2023_ICCV} and TSGAD \cite{noghre2024exploratory} models and trained them on HuVAD dataset.}
\label{tab:benchmark}
\end{table*}


\subsection{Metrics}

\textbf{AUC-ROC} gauges a model's ability to distinguish between classes at different thresholds. It calculates the area under the Receiver Operating Characteristic (ROC) curve, which plots the True Positive Rate (TPR) against the False Positive Rate (FPR) across different thresholds. Though common in VAD, AUC-ROC has drawbacks: it doesn't account for False Negative Rate (FNR), is sensitive to data imbalance, and may obscure key trade-offs by aggregating performance.

\textbf{AUC-PR}, a metric for binary classifiers that is more suited for imbalanced data. It quantifies the area under the Precision-Recall curve, summarizing classifier performance across thresholds. This metric is valuable for skewed datasets, especially when focusing on minority classes. While higher AUC-PR values signify better models, it's limited in providing detailed analysis of negative class predictions and overall error landscape.


\textbf{EER} is another measure to understand the trade-off between FPR and FNR. It shows the point where the rate of both types of errors is equal, implying a balance between sensitivity (ability to detect anomalous events) and specificity (ability to recognize normal events) in video surveillance or monitoring systems. Unlike AUC-ROC and AUC-PR, EER identifies the optimal threshold when the cost of false negatives and false positives is equal, which is especially useful for real-world deployment.


\textbf{10ER} is a metric newly introduced for VAD, based on a recent study showing that an acceptable FNR for VAD users is around 10\% \cite{ardabili2024exploring}. In line with this, we measure the FPR when the threshold is set to keep the FNR at 10\%. This concept is derived from False Match Rate 100 (FMR100), a metric used in biometric systems \cite{maio2002fvc2002} and \cite{neto2022ocfr}, where it refers to the FPR when the system maintains an FNR of 1\%.




\subsection{EP1: Standard Evaluation Protocol}

In the unsupervised learning paradigm, models are trained by minimizing a specific objective to only learn the normal behavior and then evaluated once on a test set. This approach prevents feedback or information leakage between training and evaluation, preserving the integrity of the process.


\subsection{EP2: Continual Learning Evaluation Protocol}

To simulate distribution shifts, we pre-train models on the SHT dataset \cite{liu2018future} as the static starting data and adjust HuVAD to mimic real-world streaming data for step-by-step continual training. Given that anomalies are rare in real-world settings, we start with the predefined train and test sets from the original data split (Table \ref{tab:frame-count}) and randomly incorporate anomalies into the training stream, ensuring that less than 1\% of the training data is anomalous. The test set is edited to be balanced with an approximate 1:1 ratio of normal to anomalous frames to make metrics such as AUC-ROC and AUC-PR more informative. The removed normal frames are added to the streaming training set, which is then split into 9 segments for 9 continual learning steps. We evaluate the two most recent VAD models, STG-NF \cite{Hirschorn_2023_ICCV} and TSGAD (pose branch) \cite{noghre2024exploratory}, using this framework.


\begin{figure*}
    \centering
       \includegraphics[width=1\linewidth, trim= 28 80 38 40,clip]{graph/cont.pdf}
            \caption{
                Continual learning benchmark using TSGAD (red) \cite{noghre2024exploratory} and STG-NF (blue) \cite{Hirschorn_2023_ICCV}. The dotted line represents the baseline (trained on SHT's training set \cite{liu2018future} and tested on HuVAD-C's test set), the dashed line shows normal training (conventional training method), and the solid line indicates continual learning.}
            
 \label{fig:big}
\end{figure*}

==> sec/Future.tex <==
\section{Research Questions and Future Directions}

% comprehensive metric
% real-world
% context specific
% single pose

% miltomodal diffiusion
% Incremental learning


Our study underscores the limitations of evaluating anomaly detection models with single metrics. We advocate for a comprehensive approach, introducing real-world metrics like 10ER. Our analysis of the PHEVA dataset marks a shift towards considering contextual nuances for anomaly detection. Furthermore, exploring incremental and online learning methods for adapting to dynamic environments is important. Additionally, questions persist regarding the design of comprehensive evaluation metrics for real-world scenarios as well as the impact of integrating social interaction on detection accuracy. By highlighting these areas, we seek to inspire advancements in anomaly detection, fostering the development of sophisticated solutions capable of addressing challenges in diverse contexts.

==> sec/Privacy_Full.tex <==
\section{Privacy and Ethical Considerations} \label{sec:privacy}

Integrating computer vision algorithms into various sectors of society has underscored the importance of responsibly developing these technologies, with a keen focus on privacy and ethical considerations \cite{ahmad2022developing}. In VAD and Smart Video Surveillance (SVS), the implications of AI-driven technologies extend beyond technological advancements, touching upon critical ethical concerns such as bias, discrimination, and privacy violations \cite{ardabili2022understanding}. These concerns have practical implications for the performance and fairness of computer vision systems in real-world applications. Bias in VAD algorithms can lead to discriminatory practices, where specific demographics may be unfairly targeted or misrepresented \cite{raso2018artificial, noriega2020application}. Privacy concerns are equally significant, as the pervasive monitoring and analysis of individuals without adequate safeguards can lead to unwarranted privacy invasions, raising ethical and legal issues \cite{ardabili2023understanding}.

Addressing these privacy and ethical concerns necessitates a multifaceted approach. For instance, \cite{ardabili2023understanding} proposed a four-tier system design to safeguard privacy in developing AI-driven models, aligning with privacy protection legislation. These tiers encompass the algorithm, system, model, and data levels. However, ethical considerations are particularly crucial during the dataset creation \cite{whang2023data} and algorithm development. Adopting more abstract representation techniques, such as only focusing on human pose information, has been proposed as an intermediate solution to address some of the privacy, biases, and ethical concerns if not fully mitigating them \cite{ardabili2023understanding}. Our qualitative interaction with communities also proves that the public and stakeholders are more responsive and participatory to dataset collection and algorithm development when focusing solely on human pose information rather than actual pixels. However, transitioning to a more abstract approach (human pose information rather than deep features at the pixel level) raises questions regarding the potential compromise in model accuracy. Recent advancements challenge this notion. On the SHT dataset \cite{liu2018future}, pixel-based methods like SSMTL++v2 \cite{barbalau2023ssmtl++} and Jigsaw-VAD \cite{wang2022video} achieve AUC-ROC scores of 83.80 and 84.30, while pose-based approaches like MoPRL \cite{yu2023regularity} and STG-NF \cite{Hirschorn_2023_ICCV} attain AUC-ROC scores of 83.35 and 85.90. 

Our objective is to initiate the trend of de-identifying PII at the data collection phase instead of the algorithmic phase. This methodology not only addresses legal challenges but also promotes expedited data gathering and dissemination. Such an approach is anticipated to facilitate research and technological advancements more finely attuned to the complexities of human behavior and societal requirements.




==> sec/Statistics.tex <==
\section{Comparative Dataset Analysis: Statistical Insights}
\label{sec:stat}



% In alignment with the privacy-preserving perspective as outlined in Section \ref{sec:privacy}, our dataset only provides pose sequence data, as opposed to raw pixel data. For a fair comparison, HuVAD is exclusively benchmarked against continuously recorded, large-scale, recent human-centric datasets, as elaborated in Section \ref{sec:related}. HuVAD stands as the most extensive pose-based, continuously recorded VAD dataset to date, with over five million frames (equivalent to $\sim46$ hours) with pose sequences available that are captured continuously and annotated from CCTV cameras. As detailed in Table \ref{tab:frame-count}, HuVAD offers more than 5 times the number of normal training frames as the next largest dataset. Furthermore, the dataset includes a substantial test segment comprising over 700K frames (equivalent to $\sim6.5$ hours) which is 4 times more than the second largest dataset, split into approximately 70\% of normal and 30\% of anomalous frames.


In line with the privacy-preserving approach discussed in Section \ref{sec:privacy}, our dataset exclusively provides pose sequence data rather than raw pixel data. For a fair comparison, HuVAD is benchmarked against recent, large-scale, continuously recorded unsupervised human-centric datasets. HuVAD is the largest pose-based, continuously recorded VAD dataset to date, with over five million frames ($\sim46$ hours) of annotated pose sequences from CCTV cameras. As detailed in Table \ref{tab:frame-count}, HuVAD offers over five times more normal training frames than the next largest dataset and includes a substantial test set with over 700K frames ($\sim6.5$ hours), which is four times larger than the second largest dataset, with a 70/30 split between normal and anomalous frames. \hl{Beyond the large volume of frames, the dataset's quality is highlighted by the pose count, which exceeds 8 million in the training set and nearly 1.5 million in the test set}. Figure \ref{fig:bbox_all} compares pose counts across various datasets, segmented by different views, providing a more detailed metric than frame counts alone. The large volume of per-camera data points is intentionally designed to meet the demands of emerging evaluation methods, such as online and continual learning experiments as discussed in Section \ref{sec:intro}.


% Beyond the volume of frames, the dataset's quality of the dataset is further quantified by the count of bounding boxes with a pose, referred to as the pose count. HuVAD distinguishes itself by exceeding more than 8 million poses within the training set and nearly 1.5 million poses within the test set. Figure \ref{fig:bbox_all} provide a visual comparison of pose counts across various datasets, segmented by different views. This metric underscores the volume of our dataset with more details compared to mere frame counts.


% The findings regarding S-DoM \cite{noghre2023understanding}, as presented in Table \ref{tab:sdom}, show that datasets such as SHT \cite{liu2018future} and the IITB 
% \cite{rodrigues2020multi} are characterized by positive S-DoM scores, indicating a relatively lower level of complexity. Conversely, both CHAD \cite{danesh2023chad} and HuVAD exhibit negative S-DoM values, suggesting a greater diversity within normal sequences across training and testing sets, as well as a closer similarity between normal sequences in the training set and anomalous sequences in the test set, with HuVAD being more challenging.


Figures \ref{fig:full_analyze}.A and \ref{fig:full_analyze}.B depict the distribution of the highest Intersection over Union (IoU) ratio per frame, comparing this data across different datasets and among the various cameras within the HuVAD dataset. A high IoU among bounding boxes indicates increased scene occlusion and a more challenging environment. Figure \ref{fig:full_analyze}.A highlights HuVAD's occlusion distribution compared to its peers. IITB\cite{rodrigues2020multi} and CHAD\cite{danesh2023chad} are characterized by a wide range of IoU values, which suggests variability in the level of scene occlusion. In contrast, the SHT\cite{liu2018future} dataset, much like HuVAD, maintains a smaller range of distribution. On the other hand, Figure \ref{fig:full_analyze}.B shows that HuVAD includes various levels of occlusion across all cameras. CSC stands out as the most occluded and challenging camera with the highest median.

It is also shown in Figure \ref{fig:full_analyze}.C and \ref{fig:full_analyze}.D that most of the views have a substantial density from 3 to 14 people per frame except for CSC, which shows a higher crowd density due to its nature showcasing groups of people conducting security training. CHAD \cite{danesh2023chad} exhibits the lowest range of crowdedness and SHT \cite{liu2018future} the highest. HuVAD generally stands out for its number of frames for each level of crowdedness.


